ClimateNeRF: Extreme Weather Synthesis in Neural Radiance Field

Physical simulations produce excellent predictions of weather effects. Neural radiance fields produce SOTA scene models. We describe a novel NeRF-editing procedure that can fuse physical simulations with NeRF models of scenes, producing realistic movies of physical phenomena in those scenes. Our application -- Climate NeRF -- allows people to visualize what climate change outcomes will do to them. ClimateNeRF allows us to render realistic weather effects, including smog, snow, and flood. Results can be controlled with physically meaningful variables like water level. Qualitative and quantitative studies show that our simulated results are significantly more realistic than those from SOTA 2D image editing and SOTA 3D NeRF stylization.

==> 1_introduction.tex <==
\section{Introduction}

This paper describes a novel procedure that fuses physical simulations
with NeRF models~\cite{mildenhall2020nerf, muller2022instant} of scenes to produce realistic movies of physical phenomena in those scenes.  
We apply our method to produce compelling simulations of possible extreme weather outcomes -- what would the playground look like after a minor flood?  a major flood?
a blizzard?

\input{figures/3_overview.tex}

Our application -- Climate NeRF -- is aimed at an important problem.
Cumulative small changes are hard to reason about, and most people find
it difficult to visualize what climate change outcomes will do {\em to them} ~\cite{chapman2016climate,
  glaas2017visualization, herring2017communicating, leviston2014imagining}. Steps to
slow $\mbox{CO}_2$ emissions (say, reducing fossil fuel use) or to moderate outcomes (say, building flood control
measures) come with immediate costs and distant benefits.  It is hard to support such steps if one can't visualize their
effects.  

We show how to merge \emph{physical simulations} -- which produce excellent predictions of weather effects, but only moderate images -- with \emph{neural radiance fields} -- which produce SOTA scene models but (as far as we know) have never been used
together with physical simulations.  
Traditional physical simulations can produce realistic weather effects for 3D
scenes in a conventional graphics pipeline~\cite{stomakhin2013material, feldman2002modeling, horvath2015empirical, zsolnai2022flow, blender,unrealengine, haas2014history}. 
But these methods operate on conventional polygon models.
Building polygon models that produce compelling renderings from a few images of a scene remains challenging. 
Neural radiance fields (NeRFs) produce photorealistic 3D scene models from few images~\cite{mildenhall2020nerf, barron2022mip, muller2022instant, chen2022tensorf, tancik2022block, wu2022diver, lin2022neurmips}.  
Our method draws from a large literature, reviewed below, that explores editing these models. 


ClimateNeRF allows us to render realistic weather effects, including smog, snow, and flood.  These effects are
consistent over frames, so that compelling movies result.  At a high level, we:  adjust scene images to
reflect global effects of the physics; build a NeRF model of a
scene from those adjusted images; recover an approximate geometric representation; apply the physical simulation in that
geometry; then render using a novel ray tracer.  Adjusting the images is important.  For example,
trees tend to have less saturated images in winter.  We use a novel style transfer approach in an NGP framework
to obtain these global effects without changing scene geometry (Section~\ref{sec:stylization}). 
Our ray tracer merges the physical and NeRF models by carefully accounting for ray effects during rendering (Section~\ref{sec:simulation}).  An eye ray could, for example, first encounter a high NeRF density (and so return the usual result); or it
could strike an inserted water surface (and so be reflected to query the model again).


We demonstrate the effectiveness of ClimateNeRF in various 3D scenes from the Tanks and Temple, MipNeRF360, and
KITTI-360 datasets~\cite{barron2022mip, Knapitsch2017, liao2022kitti}.  We compared to the state-of-the-art 2D image editing
methods, such as stable diffusion inpainting~\cite{rombach2021highresolution}, ClimateGAN~\cite{schmidt2021climategan};
state-of-the-art 3D NeRF stylization~\cite{zhang2022arf}.  Both qualitative and quantitative studies show that our
simulated results are significantly more realistic than the other competing methods.  Furthermore, we also demonstrate
the controllability of our physically-inspired approaches, such as changing the water level, wind strength and
direction, and thickness of snow and smog.  

Our approach results in view consistency (so we can make movies, which is difficult to do with frame-by-frame synthesis); compelling photorealism (because the scene is a NeRF representation); and is controllable (because we can adjust physically meaningful parameters in the simulation).
As Fig.~\ref{fig:1_teaser} illustrates, results are photo-realistic, physically plausible, and temporally consistent.



==> 3_method.tex <==
\input{figures/method/stylization}

\section{Method}
\label{sec:method}
\input{figures/method/flood_render}

ClimateNeRF fuses physical simulations with NeRF models of scenes to produce realistic videos of climate change
effects. A simple example illustrates how components interact in our approach.  Imagine we wish to build a model of a
flooded scene in Fall.  We acquire images, apply a Fall style (Section~\ref{sec:stylization}), and build a NeRF from the
results (Section~\ref{sec:modeling}).  We then use geometric information in that NeRF to compute a water surface.  This
is represented using a density field, a color field together with normal and BRDF representations
(Section~\ref{sec:simulation}). Finally, to render we query the model with rays.  The details are elaborate
(Section~\ref{sec:implementation}), but the general idea is straightforward:  we edit the NeRF's density
and color functions to represent effects like smog; and we intercept rays to represent specular effects.
So if a ray encounters high density in the NeRF first, we use the NeRF integral for that ray;  but if the
first collision is with the water surface, we reflect
that ray in the water surface, then query the NeRF with the reflected ray.
Fig.~\ref{fig:3_overview} provides an overview of our approach.   

\subsection{3D Scene Reconstruction}
\label{sec:modeling}


NeRF builds a parametric scene representation that supports realistic rendering from
multiple images of a scene obtained at known poses. The scene is represented by a field
\begin{equation}\label{eq:nerf_cd}
    (\sigma, \mathbf{c}) = F_{\theta}(\mathbf{x}, \mathbf{d}),
\end{equation}
which accepts position $\bx$ and direction $\bd$
and predicts density $\sigma \in \bbR$ and color 
$\mathbf{c} \in \bbR^3$. This function is encoded in a multi-layer perceptron (MLP) with learnable parameters
$\theta$.  Rendering is by querying radiance along appropriate choices of ray,
computed as a volume integral~\cite{kajiya1984ray}.  This integral is estimated
by drawing samples along the ray, evaluating the density and color at those samples,
then accumulating values.   The rendering process is differentiable, so that NeRF can be trained by minimizing the image 
reconstruction loss over training views through gradient descent: $\min_\theta \sum_{\br}\|C(\mathbf{r}) -
C_{gt}(\mathbf{r})\|_2^2$.   


There are numerous variants of NeRF. 
We use instant-NGP~\cite{muller2022instant} to reconstruct the scene. This
is an efficient NeRF alternative that explicitly stores multi-resolution features $\gamma$ for scene
representation. During rendering, given an input point, a local feature $\gamma(\bx)$ is firstly queried through a
spatial hashing function~\cite{teschner2003optimized} and is then sent to a shallow multi-layer perceptron (MLP) to
compute the final density $\sigma$ and color $\bc$: $\sigma, \bc = F_\theta(\bx, \bd; \gamma(\bx))$.  
This explicit feature encoding and spatial partition are particularly suitable for ClimateNeRF because we can
edit local features relatively easily.

A physical simulation needs access to the surface normal of any point to compute interactions with
snow and water, and it needs access to the point's semantics (in the sense of semantic segmentation) to
transfer style.  We expand the NGP and allow it to output both semantic logic $\bs$ and surface normal $\bn$. There is
no semantic or surface normal ground truth during training. We use an off-the-shelf pretrained monocular semantic
segmentation network~\cite{xie2021segformer} to produce semantic maps for each image.
We use density gradients
$\hat{\mathbf{n}}=-\frac{\nabla \sigma}{\|\nabla\sigma\|}$~\cite{boss2021nerd, srinivasan2021nerv}
(cf. Ref-NeRF~\cite{verbin2022refnerf}) to guide the predicted surface normals $\mathbf{n}$ with a weighted MSE loss.

To simulate (say) a blizzard, we must add snow to the scene and turn trees dark, but should not change the shape of the
house.  To keep spatial features intact at the stylization stage, we disentangle instant-NGP's latent feature
(as in~\cite{chen2022tensorf, sun2022direct}).   For each voxel in the NGP model, we split the latent
feature into geometry features $\gamma_\text{geo}$ and appearance features $\gamma_\text{app}$. The geometry features
are trained to render density. The appearance features are used for rendering color, semantics and normals.
We will freeze the geometry feature vector during the stylization stage and change only the appearance feature vector.  

Our 3D scene representation model \zhihao{is built on top of instant-NGP~\cite{muller2022instant}, and} renders density $\sigma$, color $\bc$, semantic log posterior $\bs$ and surface normal $\bn$, given a query point
and ray direction, so
\begin{equation}
\label{eq:ngp}
    (\sigma, \mathbf{c}, \mathbf{s}, \mathbf{n}) = F_{\theta}(\mathbf{x}, \mathbf{d}; \gamma_\text{geo} , \gamma_\text{app})
\end{equation}
\zhihao{The non-ideal geometry in neural scene~\cite{mildenhall2020nerf, muller2022instant} generates severe artifacts in the simulation. To this end, per-frame appearance embedding~\cite{martin2021nerf} and distortion loss~\cite{barron2022mip} are adopted to remove floaters. Furthermore, the normal MLP makes scene normal smooth spatially, and novel sky loss $\mathcal{L}_{\text{sky}}=\sum_{\br \in \text{sky}}e^{-d(\br)}$ is proposed to increase depth and remove floaters in sky region. The improved geometry boosts simulation realism significantly.}

(more details in supplementary).

\input{figures/method/snow_render}


\subsection{Stylization}
\label{sec:stylization}

Deciduous trees drop their leaves in winter, and physical simulation is not an efficient way to capture effects like this.
We use FastPhotoStyle~\cite{li2018closed} to transfer style to rendered images from a pre-trained model $F_{\theta}$. 
We only transfer only to regions 'terrain', 'vegetation', or 'sky' regions
to mimic natural weather change phenomena.
The resulting images look realistic but are not necessarily view-consistent. Hence, a student instant-NGP model is fined-tuned to ensure the view consistency of the style-transferred scene.  This is trained to minimize the color difference between our student NeRF-rendered results and style-transferred images. %
We  keep the geometry intact and alter only  appearance to achieve this goal, so only the appearance feature code $\gamma_\text{app}$ is optimized during the style transfer stage: 
\begin{equation}\label{eq:stylize_loss}
    \min_{\gamma_\text{app}} \sum_{\mathbf{r} \in \mathcal{R}}\left\|C(\mathbf{r})-C_\text{stylized}(\mathbf{r})\right\|_{2}^{2} 
\end{equation}
where $C(\br)$ is renderd color and $C_\text{stylized}$ is the style-transferred in the same view. This gives us a new NGP model $(\sigma, \mathbf{c}') = F_{\theta}'(\mathbf{x}, \mathbf{d}, \ell^{(a)}_{i})$ which encodes the style. Fig.~\ref{fig:4_stylization} demonstrates the visual effects of such NeRF stylization.
This optional style transfer step simulates composite effects, such as a flood in Fall,  where the original
images were captured in Spring.

\subsection{Representing and Rendering Climate Effects}\label{sec:simulation}

We want to generate scenes with new physical entities -- snow, water, smog -- in place.  We must
determine where they are (the job of physical simulation) and what the resulting image looks like (the job of
rendering).   {\em How} the simulation represents results is important, because results must be accessible to the
rendering process.  Rendering will always involve computing responses to ray queries, so computing
radiance at $\mathbf{u}$ in direction $\mathbf{v}$.
We must represent simulation results in terms of densities and we must be able to compute normals and surface
reflectance properties.  Generally, we write $O_{\phi}(\bx; F_{\theta}): \bbR^3 \rightarrow \bbR$ for a density
resulting from a physical simulation; $N_\phi(\bx; F_{\theta}): \bbR^3 \rightarrow \bbS^2$ for normals;
and $B_\phi(\bx, \bomega_o, \bomega_i; F_{\theta}): \bbR^9 \rightarrow \bbR$ for BRDF.  Each depends on the existing
scene $F_\theta$. Choice of $B_\phi$ can simulate various effects, including the atmospheric effect of smog, refraction
and reflections on water surfaces, and scattering of accumulated snow.  
$\{O_\phi, N_\phi, B_\phi\}$ differs drastically across different physical simulations (details per effect in Sect.~\ref{sec:implementation}).

Once the physical entities are defined by functions $O_{\phi}, N_\phi, B_\phi$, we can render them realistically into
the image by modeling the light transport between the physical entities and the scene.    Given the query point position
$\bx$, the simulation framework estimates the density and color of physical entities at position $\bx$ through
physically based rendering: 
\begin{equation}
\label{eq:unify_cd_physical}
\begin{split}
    \sigma_{\phi} &= O_{\phi}(\mathbf{x}; F_{\theta}), \\
    \mathbf{c}_{\phi} &= \int_{\Omega} L(\mathbf{x}, \bomega_i)B_{\phi}(\mathbf{x}, \mathbf{d}, \bomega_i; F_{\theta})(\bomega_i \cdot N_\phi(\bx; F_{\theta})) \text{d}\bomega_i,
\end{split}
\end{equation}
where entity color $\bc_{\phi}$ is approximated with physically-based rendering equation~\cite{kajiya1986rendering} with
normal $N_\phi$ and BRDF $B_\phi$.  Importantly, we approximate the incident illumination $L(\bx, \bomega_i)$ with
radiance by tracing a ray $\br(t) = \bx-t\bomega_i$ opposite to the incident direction in the learned NeRF, \ie $L(\bx,
\bomega_i) = C(\br)$.  %
Depending on the surface BRDF of physical entities, we use analytical or sampling-based solutions for the integral. Note
that multiple bounces can be simulated through sampling.   

We follow the volumetric rendering process defined in two passes. For every point along a camera ray, we query the opacity and color of the physical entities as defined in Eq.~\ref{eq:unify_cd_physical}. In the meantime, the system also retrieves the original density $\sigma_{\theta}$ and color $\bc_\theta$ through Eq.~\ref{eq:ngp}. \method~estimates final density and color of the simulated scene by:
\begin{equation}\label{eq:unify_cd}
     {\sigma}_\text{final} = \sigma_{\theta} + \sigma_{\phi}, \quad
     \bc_\text{final}= \frac{\sigma_{\theta}\mathbf{c}_{\theta} + \sigma_{\phi}\mathbf{c}_{\phi}}{\sigma_{\theta} + \sigma_{\phi}},
\end{equation}
Once ${\sigma}_\text{final}, \bc_\text{final}$ are estimated for each ray points $\{\mathbf{x}_i\}$, the pixel color is
calculated by volume rendering.
Fig.~\ref{fig:3_rendering} depicts the entire physically
inspired simulation and rendering process.  
\input{tables/4_quality_smog.tex}
\input{tables/4_quality_flood.tex}
\input{figures/refraction}

\subsection{Climate Effect Details}
\label{sec:implementation}

\method~is able to simulate smog, flood, and snow through various choices of $\{O_{\phi}, N_\phi, B_\phi \}$.
\paragraph{Smog Simulation} We assume that smog is formed by tiny absorbing particles, uniformly distributed
in empty space.  In empty space the NeRF density $\sigma_{\theta}=0$.  The Beer-Lambert law (originally~\cite{beer,
  lambert}; in~\cite{fox}) means we can model smog density in free space by simply adding a non-negative constant
to the density.  Inside high density regions of the NeRF, adding the constant does not significantly change the
integral, so we have
\begin{equation}
  O_\phi(\bx; F_\theta)   = \sigma_{\text{smog}} 
\end{equation}
where $\sigma_\phi$ is a controllable parameter that decides the density of the smog. Smog particles have
a constant color $\bc_{\text{smog}}$.  Both $\bc_\text{smog}$ and $\sigma_{\text{smog}}$ are controllable
parameters. Fig.~\ref{tab:4_control} depicts the effects of various smog densities.  

\paragraph{Flood Simulation}

The water surface of the flooded scene is approximately a horizontal plane: $\bn_w(\bx - \bo_w) = 0$, where the gravity
direction normal $\bn_w$ is estimated with camera poses and vanishing points detection~\cite{lu20172}, and plane origin
$\bo_w=(0, 0, h)$ determines the water height. But there are water ripples, which we implement
following~\cite{horvath2015empirical} with Fast Fourier Transform (FFT) based ripples and waves. The
FFT wave takes random spectral coefficients as input and outputs a spatiotemporal surface normal based on wind speed,
direction, and spatial and temporal frequencies. As shown in Fig.~\ref{tab:4_quality_flood}, compared against still water,
FFT-based water surface simulation significantly improves the realism of the water surfaces. We simulate opacity and
micro-facet ripples that make the water look glossy (details in supplementary).
 To approximate the integral in Eq.~\ref{eq:unify_cd_physical}, we adopt the sigma-point
method~\cite{menegaz2015systematization, wan2000unscented} and sample 5 rays from $\bx$, including reflection direction
$\bd_r$ and nearby four rays.    \method~simulates Fresnel effect, glossy reflection, and wave dynamics.



\paragraph{Snow Simulation}
Snow is more likely to be accumulated on surfaces facing upward, and the deeper part of the snow is denser due to
gravity. We simulate density distributions over %
object surfaces using metaballs~\cite{nishita1997modeling, keselman2022fuzzy} centered on surfaces and with density
$\sigma_o$ at the center. \yuan{We further simulate geometry occlusions along snow falling direction and finetune $\sigma_o$ by calculating transparency in volume rendering.} The density distribution within a metaball can be formulated by kernel function $\mathbf{K}(r,
R, \sigma_o)$, which leads to a smooth decrease of density as the distance $r$ from the metaball's center grows.   
We follow~\cite{van2007point} and tuned it to create a denser visual effect: 
$
    \mathbf{K}(r, R, \sigma)=\frac{315}{64\pi1.5^7}(1.5^2-(\frac{r}{R})^2)^3\sigma  
    $

For any point $\mathbf{x}$ in the space, we calculate the snow's density of $\mathbf{x}$ using a parzen window density
estimator over $N$ local nearest neighbors (details in supplementary).   The final density of the snow surface is decided accordingly:
\begin{equation}\label{eq:snow_density_final}
    O_\phi(\bx; F'_\theta) = 
    \frac{1}{1+e^{-a(x\sigma_{\text{snow}}-\tau_\text{snow})}} \sigma_{\text{snow}},
\end{equation}
where $\tau_\text{snow}$ is a controllable surface truncation threshold {and $a$ is a hyper-parameter}. This equation implies a point is more likely to be surface boundary if it's close or larger than the threshold.  
We use a spatially-varying diffuse color $\mathbf{c}_\phi(\bx_i^{(p)})$ (which is close to pure white
multiplied by the average illumination of the scene) to approximate BRDF,
and apply a subsurface scattering effect~\cite{nishita1997modeling} to light the snow's shadowed part (further detail in
supplementary). \yuan{We cast shadows on snow by calculating visibility along user-defined sun direction.} Surface normal values are still calculated in a gradient based manner. A visualization of snow rendering is shown in Fig.~\ref{tab:snow_render}.


